Diffusion Handles: Enabling 3D Edits for Diffusion Models by Lifting Activations to 3D

Diffusion Handles is a novel approach to enabling 3D object edits on diffusion images. We accomplish these edits using existing pre-trained diffusion models, and 2D image depth estimation, without any fine-tuning or 3D object retrieval. The edited results remain plausible, photo-real, and preserve object identity. Diffusion Handles address a critically missing facet of generative image based creative design, and significantly advance the state-of-the-art in generative image editing. Our key insight is to lift diffusion activations for an object to 3D using a proxy depth, 3D-transform the depth and associated activations, and project them back to image space. The diffusion process applied to the manipulated activations with identity control, produces plausible edited images showing complex 3D occlusion and lighting effects. We evaluate Diffusion Handles: quantitatively, on a large synthetic data benchmark; and qualitatively by a user study, showing our output to be more plausible, and better than prior art at both, 3D editing and identity control. Project Webpage: https://diffusionhandles.github.io/

==> sec/3_background.tex <==
\section{Background}

\subsection{Diffusion Generative Models}

\begin{itemize}
    \item Basic diffusion background: Diffusion models learn to transform random noise to high-resolution images. They achieve this by learning to reverse a sequential sampling process where data is corrupted by iteratively adding noise. The diffusion model iteratively denoises a given noisy sample $z_t$ by learning a neural network $\epsilon_{\theta}$ that aims to predict the initial noise $\epsilon_{t}$ that was added to corrupt the original sample at timestep $t$. 
\end{itemize}

\begin{itemize}
    \item Text-to-image generation: In the presence of additional conditional input $y$ such text, $\epsilon_{\theta}$ typically has a U-Net architecture with cross and self-attentions at multiple resolutions to attend to the conditioning signal. In this case, $\epsilon_{\theta}$ is trained with the following loss.  
\end{itemize}

\begin{equation}
    L(\theta) = \mathbb E_{t \sim U(1,T), \epsilon_t \sim \mathcal{N}(0, \textbf{I})} [ \left \lVert \epsilon_t - \epsilon_{\theta} (z_t; t;y) \right \rVert ]
\end{equation}

\begin{itemize}
    \item Denoising process: The denoising process then consists of iteratively estimating the noise at a given timestep, and updating the noisy image. In particular, it can be expressed as the following update, where $\hat{\epsilon_t}$ is the predicted noise used in the update function to perform a denoising step at timestep $t$. 
\end{itemize}

\begin{equation}
    \hat{\epsilon_t} = \epsilon_{\theta} (z_t; t;y), z_{t-1} = \text{denoiser} (z_t, \hat{\epsilon_t}, t), 
\end{equation}

%so basically we want to introduce enough to introduce the guidance notation 
%guidance has y, 

\subsection{Guidance}

\begin{itemize}
    \item Diffusion models allow for steering the generation process at inference time by guiding the sampling process based on a supplied energy. In particular, the noise prediction step earlier can be augmented as follows to incorporate guidance.
    %This has been used to accomplish a number of  
\end{itemize}

\begin{equation}
\label{eq:guidance}
    \hat{\epsilon_t} = (1 + s) \epsilon_{\theta} (z_t; t;y) - s \epsilon_{\theta} (z_t; t;\emptyset) + w \nabla_{z_t} g (z_t; t;y) 
\end{equation}

\begin{itemize}
    \item - The classifier-free guidance term $\epsilon_{\theta} (z_t; t;\emptyset)$ is used to maintain the diffusion models prior ability to generate high-quality images across guidance. \\
    - The energy term $g$ is the energy we want to minimize with the guidance. In previous work, $g$ has been defined as a function of the cross-attention maps and activations of the U-Net denoiser's decoder to control the layout and appearance of elements in the generated scene. In particular, prior work has found that cross attention maps are related to the structure / layout of the generated scene and the activations encode coarse appearance. 
\end{itemize}


%\begin{itemize}
%    \item Establish notation
%    \item Describe vanilla and depth-conditioned text-to-image models
%    \item Describe self-guidance loss
%\end{itemize}
